Energy-aware Multi-UAV Coverage Mission Planning with Optimal Speed of Flight

This paper tackles the problem of planning minimum-energy coverage paths for multiple UAVs. The addressed Multi-UAV Coverage Path Planning (mCPP) is a crucial problem for many UAV applications such as inspection and aerial survey. However, the typical path-length objective of existing approaches does not directly minimize the energy consumption, nor allows for constraining energy of individual paths by the battery capacity. To this end, we propose a novel mCPP method that uses the optimal flight speed for minimizing energy consumption per traveled distance and a simple yet precise energy consumption estimation algorithm that is utilized during the mCPP planning phase. The method decomposes a given area with boustrophedon decomposition and represents the mCPP as an instance of Multiple Set Traveling Salesman Problem with a minimum energy objective and energy consumption constraint. The proposed method is shown to outperform state-of-the-art methods in terms of computational time and energy efficiency of produced paths. The experimental results show that the accuracy of the energy consumption estimation is on average 97% compared to real flight consumption. The feasibility of the proposed method was verified in a real-world coverage experiment with two UAVs.

==> tbl/single_target_success.tex <==
%!TEX root = ../main.tex 
\begin{table}[t] 
   \centering 
   \footnotesize 
   {\renewcommand{\tabcolsep}{3.0pt} 
   %\renewcommand{\arraystretch}{0.6} 
   \caption{Comparison of success rates of navigating through waypoints while avoiding obstacles.\label{tab:success}} 
   \vspace{-1em} 
   \begin{tabular}{lcrrrrrr}
     \toprule 
    \multirow{2}{*}{Env.} & \multirow{2}{*}{\begin{minipage}{5mm}Test\\case\end{minipage}} & \multicolumn{3}{c}{SB~\cite{penicka22RALsbmintimequad} + MPC~\cite{foehn2020cpc}} & \multicolumn{3}{c}{\textbf{RL (ours)}} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8}                            &                            & success[\%] & $T_{a}$[s] & $T_{b}$[s] & success[\%]  & $T_{a}$[s] & $T_{b}$[s]\\ 
     \midrule 
\multirow{4}{*}{Forest} & 0 & 25 & \textbf{1.22} & \textbf{1.13} & \textbf{100} & 1.23 & 1.21\\ 
& 1 & 0 & \textbf{-} & - & \textbf{100} & \textbf{1.21} & \textbf{1.18}\\ 
& 2 & 27 & \textbf{1.14} & \textbf{1.11} & \textbf{100} & 1.20 & 1.18\\ 
& 3 & 16 & 1.70 & \textbf{1.42} & \textbf{100} & \textbf{1.57} & 1.56\\ 
\midrule 
\multirow{4}{*}{Office} & 0 & 41 & 2.38 & 2.12 & \textbf{100} & \textbf{1.91} & \textbf{1.89}\\ 
& 1 & 28 & 1.86 & \textbf{1.78} & \textbf{100} & \textbf{1.84} & 1.82\\ 
& 2 & 56 & 2.29 & 1.97 & \textbf{100} & \textbf{1.74} & \textbf{1.72}\\ 
& 3 & 70 & 2.16 & \textbf{1.70} & \textbf{100} & \textbf{1.99} & 1.96\\ 
\midrule 
\multirow{4}{*}{Racing} & 0 & 57 & 1.61 & 1.46 & \textbf{100} & \textbf{1.41} & \textbf{1.39}\\ 
& 1 & 51 & 1.64 & 1.45 & \textbf{100} & \textbf{1.47} & \textbf{1.44}\\ 
& 2 & 76 & 1.72 & 1.51 & \textbf{100} & \textbf{1.51} & \textbf{1.49}\\ 
& 3 & 54 & 1.80 & 1.62 & \textbf{100} & \textbf{1.46} & \textbf{1.43}\\ 
\midrule 
\multirow{1}{*}{Racing MW} & 0 & 25 & \textbf{7.22} & \textbf{7.17} & \textbf{100} & \textbf{7.22} & 7.18\\ 
\bottomrule 
   \end{tabular} 
   } 
   \vspace{-1.0em}
\end{table} 



